Deep Q-Network-based Adaptive Alert Threshold Selection Policy for Payment Fraud Systems in Retail Banking

Machine learning models have widely been used in fraud detection systems. Most of the research and development efforts have been concentrated on improving the performance of the fraud scoring models. Yet, the downstream fraud alert systems still have limited to no model adoption and rely on manual steps. Alert systems are pervasively used across all payment channels in retail banking and play an important role in the overall fraud detection process. Current fraud detection systems end up with large numbers of dropped alerts due to their inability to account for the alert processing capacity. Ideally, alert threshold selection enables the system to maximize the fraud detection while balancing the upstream fraud scores and the available bandwidth of the alert processing teams. However, in practice, fixed thresholds that are used for their simplicity do not have this ability. In this paper, we propose an enhanced threshold selection policy for fraud alert systems. The proposed approach formulates the threshold selection as a sequential decision making problem and uses Deep Q-Network based reinforcement learning. Experimental results show that this adaptive approach outperforms the current static solutions by reducing the fraud losses as well as improving the operational efficiency of the alert system.

==> Makefile <==
MAIN=main
BIB=bib
OUTPUT_DIR=output
AUX_DIR=output_aux

.PHONY: all check link clean travis data tatoeba

pdf:
	latexmk -pdf $(MAIN) -auxdir=$(OUTPUT_DIR) -outdir=$(OUTPUT_DIR)

all: pdf
	make -C code/programs

check:
	chktex -n1 -n2 -n3 -n8 -n11 -n12 -n13 -n14 -n26 -n34 -n33 -n36 -n40 -n44 $(MAIN)
	biber --tool -V $(BIB).bib
	rm -f $(BIB)_bibertool.bib

lint:
	biber --tool $(BIB).bib --output-fieldcase=lower --isbn-normalise
	mv $(BIB)_bibertool.bib $(BIB).bib

arxiv: pdf
	mkdir -p arxiv
	cp *.pdf $(OUTPUT_DIR)/*.bbl *.bib *.tex *.cls *.bst arxiv
	#Download any new versions of packages here
	#e.g.
	#curl -L -o arxiv/algorithm2e.sty https://ctan.sharelatex.com/tex-archive/macros/latex/contrib/algorithm2e/tex/algorithm2e.sty
	#Test build
	cd arxiv && latexmk -pdf $(MAIN) -auxdir=arxivtest -outdir=arxivtest && rm -rf arxivtest
	cd arxiv && zip arxiv.zip *

clean:
	latexmk -c -pdf
	rm -rvf *.bbl *.blg *.aux *.fls *.fdb_latexmk *.log *.out *.toc $(MAIN).pdf $(AUX_DIR) $(OUTPUT_DIR) arxiv

travis:
	#Old latexmk doesn't understand auxdir and outdir options
	latexmk -pdf -pdflatex='pdflatex %S %O -interaction=nonstopmode -halt-on-error' $(MAIN)

######################
# Download data
######################
TATOEBA_CORPUS = data/tatoeba/users_sentences.csv \
	data/tatoeba/user_languages.csv \
data/tatoeba/sentences_in_lists.csv \
data/tatoeba/links.csv \
data/tatoeba/tags.csv \
data/tatoeba/sentences_detailed.csv \
data/tatoeba/user_lists.csv

data: $(TATOEBA_CORPUS)

tatoeba: $(TATOEBA_CORPUS)

data/tatoeba/users_sentences.csv:
	curl --create-dirs -R -L -z $@ -o $@ https://downloads.tatoeba.org/exports/users_sentences.csv

data/tatoeba/%.csv: data/tatoeba/%.tar.bz2
	tar -xjvf $< -C data/tatoeba

data/tatoeba/%.tar.bz2:
	curl --create-dirs -R -L -z $@ -o $@ https://downloads.tatoeba.org/exports/$(notdir $@)



==> latexmkrc <==
# Set time zone
# Reference
# https://www.overleaf.com/learn/latex/Articles/How_to_use_latexmkrc_with_Overleaf:_examples_and_techniques
$ENV{'TZ'}='America/New_York';

# Put all the style files here
# Reference
# https://www.overleaf.com/learn/latex/Questions/I%20have%20a%20lot%20of%20.cls,%20.sty,%20.bst%20files,%20and%20I%20want%20to%20put%20them%20in%20a%20folder%20to%20keep%20my%20project%20uncluttered.%20But%20my%20project%20is%20not%20finding%20them%20to%20compile%20correctly
$ENV{'TEXINPUTS'}='./styles//:' . $ENV{'TEXINPUTS'};


# The rest of the file below is copied from
# https://www.overleaf.com/learn/how-to/How_does_Overleaf_compile_my_project%3F
# as of 2019-08-23.

###############################
# Post processing of pdf file #
###############################

# assume the jobname is 'output' for Overleaf v2
my $ORIG_PDF_AGE = -M "output.pdf"; # get age of existing pdf if present

END {
    my $NEW_PDF_AGE = -M "output.pdf";
    return if !defined($NEW_PDF_AGE); # bail out if no pdf file
    return if defined($ORIG_PDF_AGE) && $NEW_PDF_AGE == $ORIG_PDF_AGE; # bail out if pdf was not updated
    my $QPDF = "/usr/bin/qpdf";
    return if ! -x $QPDF; # check that qpdf exists
    my $status = system($QPDF, "--linearize", "output.pdf", "output.pdf.opt");
    my $exitcode = ($status >> 8);
    print "qpdf exit code=$exitcode\n";
    # qpdf returns 0 for success, 3 for warnings (output pdf still created)
    return if !($exitcode == 0 || $exitcode == 3);
    print "Renaming optimised file to output.pdf\n";
    rename("output.pdf.opt", "output.pdf");
}

##############
# Glossaries #
##############
add_cus_dep( 'glo', 'gls', 0, 'glo2gls' );
add_cus_dep( 'acn', 'acr', 0, 'glo2gls');  # from Overleaf v1
sub glo2gls {
	system("makeglossaries $_[0]");
}

#############
# makeindex #
#############
@ist = glob("*.ist");
if (scalar(@ist) > 0) {
        $makeindex = "makeindex -s $ist[0] %O -o %D %S";
}

################
# nomenclature #
################
add_cus_dep("nlo", "nls", 0, "nlo2nls");
sub nlo2nls {
	system("makeindex $_[0].nlo -s nomencl.ist -o $_[0].nls -t $_[0].nlg");
}

#########
# Knitr #
#########
my $root_file = $ARGV[-1];

add_cus_dep( 'Rtex', 'tex', 0, 'rtex_to_tex');
sub rtex_to_tex {
    do_knitr("$_[0].Rtex");
}

sub do_knitr {
    my $dirname = dirname $_[0];
    my $basename = basename $_[0];
    system("Rscript -e \"library('knitr'); setwd('$dirname'); knit('$basename')\"");
}

my $rtex_file = $root_file =~ s/\.tex$/.Rtex/r;
unless (-e $root_file) {
	if (-e $rtex_file) {
		do_knitr($rtex_file);
	}
}

##########
# feynmf #
##########
push(@file_not_found, '^feynmf: Files .* and (.*) not found:$');
add_cus_dep("mf", "tfm", 0, "mf_to_tfm");
sub mf_to_tfm { system("mf '\\mode:=laserjet; input $_[0]'"); }

push(@file_not_found, '^feynmf: Label file (.*) not found:$');
add_cus_dep("mf", "t1", 0, "mf_to_label1");
sub mf_to_label1 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t1"); }
add_cus_dep("mf", "t2", 0, "mf_to_label2");
sub mf_to_label2 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t2"); }
add_cus_dep("mf", "t3", 0, "mf_to_label3");
sub mf_to_label3 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t3"); }
add_cus_dep("mf", "t4", 0, "mf_to_label4");
sub mf_to_label4 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t4"); }
add_cus_dep("mf", "t5", 0, "mf_to_label5");
sub mf_to_label5 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t5"); }
add_cus_dep("mf", "t6", 0, "mf_to_label6");
sub mf_to_label6 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t6"); }
add_cus_dep("mf", "t7", 0, "mf_to_label7");
sub mf_to_label7 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t7"); }
add_cus_dep("mf", "t8", 0, "mf_to_label8");
sub mf_to_label8 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t8"); }
add_cus_dep("mf", "t9", 0, "mf_to_label9");
sub mf_to_label9 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t9"); }

##########
# feynmp #
##########
push(@file_not_found, '^dvipdf: Could not find figure file (.*); continuing.$');
add_cus_dep("mp", "1", 0, "mp_to_eps");
sub mp_to_eps {
    system("mpost $_[0]");
    return 0;
}

#############
# asymptote #
#############
sub asy {return system("asy --offscreen '$_[0]'");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

#############
# metapost  #  # from Overleaf v1
#############
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}

##########
# chktex #
##########
unlink 'output.chktex' if -f 'output.chktex';
if (defined $ENV{'CHKTEX_OPTIONS'}) {
    use File::Basename;
    use Cwd;

    # identify the main file
    my $target = $ARGV[-1];
    my $file = basename($target);

    if ($file =~ /\.tex$/) {
	# change directory for a limited scope
	my $orig_dir = cwd();
	my $subdir = dirname($target);
	chdir($subdir);
	# run chktex on main file
	$status = system(
    "/usr/bin/run-chktex.sh",
    $orig_dir,
    $file
  );
	# go back to original directory
	chdir($orig_dir);

	# in VALIDATE mode we always exit after running chktex
	# otherwise we exit if EXIT_ON_ERROR is set

	if ($ENV{'CHKTEX_EXIT_ON_ERROR'} || $ENV{'CHKTEX_VALIDATE'}) {
	    # chktex doesn't let us access the error info via exit status
	    # so look through the output
	    open(my $fh, "<", "output.chktex");
	    my $errors = 0;
	    {
		local $/ = "\n";
		while(<$fh>) {
		    if (/^\S+:\d+:\d+: Error:/) {
			$errors++;
			print;
		    }
		}
	    }
	    close($fh);
	    exit(1) if $errors > 0;
	    exit(0) if $ENV{'CHKTEX_VALIDATE'};
	}
    }
}

